The dark side of the proton

We study the sensitivity of the High-Luminosity LHC to a light baryonic dark photon B, primarily coupled to quarks, as a constituent of the proton. This is achieved by allowing for a dark photon parton distribution function (PDF) in the PDF evolution equations. Depending on the mass and coupling of the dark photon, the evolution of standard quark and gluon PDFs is distorted to varying degrees. By analysing the effect of the dark photon on the tails of Drell-Yan invariant mass distributions, we demonstrate the potential of the LHC in determining competitive bounds on dark photon parameter space.

==> sec-split.tex <==
\section{Calculating splitting functions}
\label{app:splitting}
In this Appendix, we remind the reader of how to compute
(leading order) splitting functions, in the context of the calculation of the
dark photon splitting functions.

In general, a cross section for a partonic process at next-to-leading
order in some constant $\alpha$ involving the
radiation of a parton will be of the form:
\begin{equation*}
\sigma^{\text{NLO}} = \frac{\alpha}{2\pi} \int \frac{d(|\vec{l}_T|^2)}{|\vec{l}_T|^2} \int\limits_{0}^{1} \frac{dx}{1-x} P(x) \sigma^{\text{Born}}(xp) + \text{terms that remain finite as $\vec{l}_T \rightarrow 0$},
\end{equation*}
\noindent where $\sigma^{\text{Born}}(xp)$ is the cross-section when such a parton is not radiated. Here, $\vec{l}_T$ is the transverse momentum of the radiated parton and $x$ is the fraction of momentum of the parton that goes on to take part in the hard reaction. The factor $P(x)$ is called the \textit{splitting function} and depends on the type of parton initiating the process, the type of parton radiated, and the type of parton that goes on to participate in the hard reaction. It multiplies the most collinearly divergent part of the cross-section.

We now calculate the $B$-boson splitting functions at leading order explicitly. We spell out the first calculation in detail, the second is fairly similar, and the last two can be computed using probability arguments.
\subsubsection*{Contribution to $P_{qq}(x)$}
\noindent Consider a general leading order partonic process where a quark $q$ scatters off another particle $k$ (not even necessarily a parton) to produce some final state $X$ via some unknown interaction, as shown in the figure below.
\begin{figure}[H]
\centering
\begin{tikzpicture}
\begin{scope}[thick, decoration={
    markings,
    mark=at position 0.5 with {\arrow{>}}}
    ] 
\draw[postaction={decorate}] (-1,-1) node[below left] {$q$}-- (0,0);
\draw[dashed,postaction={decorate}] (-1,1) node[above left] {$k$}-- (0,0);
\end{scope}
\node[circle,fill=black,inner sep=0pt,minimum size=15pt] at (0,0) {};
\begin{scope}[ultra thick,decoration={
    markings,
    mark=at position 0.7 with {\arrow{>}}}
    ] 
\draw[postaction={decorate}] (0,0) -- (1,0) node[right] {$X$};
\end{scope}
\end{tikzpicture}
\end{figure}
\noindent The amplitude for this process can be written in the form:
\begin{equation*}
\mathcal{M}(p) u(p),
\end{equation*}
\noindent where $\mathcal{M}(p)$ is the amplitude for the unknown hard scattering part of the diagram (taking as an argument the four-momentum $p$ of our incoming quark $q$), including the final state $X$ and the target particle $k$, and $u(p)$ comes from the initial quark $q$. This amplitude gives rise to a cross-section:
\begin{equation*}
\sigma^{\text{Born}}(p) = \sum_{X} \frac{1}{2}\sum_{\substack{\text{initial} \\ \text{spins}}}\frac{1}{\mathcal{F}} \mathcal{M}(p) u(p) \bar{u}(p) \mathcal{M}^{\dagger}(p),
\end{equation*}
\noindent where the sum over $X$ includes an integral over the phase space of the final state $X$. The flux factor $\mathcal{F}$ is given by $\mathcal{F} = 4 p \cdot p' = 2s$, where $p'$ is the four-momentum of the target particle $k$, and $s$ is the usual Mandelstam variable $s = (p+p')^2$. Performing the sum over spins using the outer product spinor identity, we are left with
\begin{equation*}
\sigma^{\text{Born}}(p) = \frac{1}{4s} \sum_{X}  \mathcal{M}(p) \slashed{p} \mathcal{M}^{\dagger}(p).
\end{equation*}
\noindent Our initial quark $q$ may also radiate a $B$-boson before it participates in the interaction. Therefore, we will also get contributions from diagrams of the form:
\begin{figure}[H]
\centering
\begin{tikzpicture}
\begin{scope}[thick,decoration={
    markings,
    mark=at position 0.5 with {\arrow{>}}}
    ] 
\draw[dashed,postaction={decorate}] (-1,1) node[above left] {$k$}-- (0,0);
\end{scope}
\draw[thick,snake it] (-1.1,-1.1) -- (0.5,-1.1) node[right]{$B$};
\begin{scope}[thick,decoration={
    markings,
    mark=at position 0.7 with {\arrow{>}}}
    ] 
\draw[postaction={decorate}] (-1.5,-1.5) node[below left] {$q$}-- (0,0);
\end{scope}
\node[circle,fill=black,inner sep=0pt,minimum size=15pt] at (0,0) {};
\begin{scope}[ultra thick,decoration={
    markings,
    mark=at position 0.7 with {\arrow{>}}}
    ] 
\draw[postaction={decorate}] (0,0) -- (1,0) node[right] {$X$};
\end{scope}
\end{tikzpicture}
\end{figure}
\noindent Let $l$ be the momentum of the outgoing $B$-boson. Then the amplitude for this diagram is:
\begin{equation*}
\mathcal{M}(p-l) \frac{i}{\slashed{p} - \slashed{l}} \left(-\frac{ig_B}{3}\right) \slashed{\epsilon}(l) u(p) = \frac{g_B}{3(p-l)^2} \mathcal{M}(p-l) (\slashed{p} - \slashed{l}) \slashed{\epsilon}(l) u(p),
\end{equation*}
\noindent where $g_B/3$ is the baryonic $B$-boson coupling to all quarks, and $\mathcal{M}(p-l)$ is the same amplitude for the hard subgraph above, but this time with momentum $p-l$ entering the graph.

%%%%%%%%%%%
In the collinear limit we are interested in, we can simplify this amplitude. We shall begin by writing $l$ in terms of its \textit{Sudakov decomposition}
\begin{equation*}
l = (1-x)p + l_T + a \eta,
\end{equation*}
\noindent where $l_T$ is some transverse four-vector, $\eta$ is a null vector satisfying $2 \eta \cdot p = 1$, and $a$, $x$ are constants chosen to make the decomposition true. To see that such a decomposition really exists, we can pick a frame - for example, choose
\begin{equation*}
p = \begin{pmatrix} p^0 \\ 0 \\ 0 \\ p^0 \end{pmatrix}, \qquad l_T = \begin{pmatrix} 0 \\ l^1_T \\ l^2_T \\ 0\end{pmatrix}, \qquad \eta = \begin{pmatrix} 1/4p^0 \\ 0 \\ 0\\ - 1/4p^0\end{pmatrix}.
\end{equation*}
\noindent Then the vector $l$ can be written in this frame as:
\begin{equation*}
l = \begin{pmatrix} l^0 \\ l^1 \\ l^2 \\ l^3 \end{pmatrix} = \begin{pmatrix} (1-x)p^0 + a/4p^0 \\ l_T^1 \\ l_T^2 \\ (1-x)p^0 - a/4p^0\end{pmatrix}.
\end{equation*}
\noindent In particular, we see that choosing $x$, $p$ and $l_T$ appropriately, we can always construct this decomposition. We can determine the constant $a$ in terms of the constant $x$ by using the fact that $l$ must be on-shell:
\begin{equation*}
0  = l^2 = l_T^2 + (1-x)a \qquad \Rightarrow \qquad a = \frac{|\vec{l}_T|^2}{1-x},
\end{equation*}
\noindent where we have also used the fact that $p \cdot l_T = \eta \cdot l_T = p^2 = \eta^2 = 0$. Thus we see the Sudakov decomposition of the vector $l$ is given by:
\begin{equation*}
l = (1-x)p + l_T + \frac{|\vec{l}_T|^2}{1-x} \eta.
\end{equation*}
%
In particular, we see that as $l_T \rightarrow 0$, we have $l \rightarrow (1-x)p$, i.e. the initial and radiated partons become collinear. Thus in this notation, the collinear limit is $l_T \rightarrow 0$.
%\noindent Turning back to the amplitude, we see that there are two locations where the factor $p-l$ occurs. The Sudakov decomposition shows us that we can write this factor as:
%\begin{equation*}
%p - l = xp - l_T - \frac{|\vec{l}_T|^2}{1-x} \eta,
%\end{equation*}
%\noindent and hence
%\begin{equation*}
%(p-l)^2 = l_T^2 - \frac{|\vec{l}_T|^2 x}{1-x} = -\frac{|\vec{l}_T|^2}{1-x}.
%\end{equation*}
%\noindent
We can thus write the amplitude in the form:
\begin{equation*}
-\frac{g_B (1-x)}{3 |\vec{l}_T|^2} \mathcal{M}(p-l) \left(x \slashed{p} - \slashed{l}_T - \frac{|\vec{l}_T|^2}{1-x}\slashed{\eta} \right) \slashed{\epsilon}(l) u(p).
\end{equation*}
\noindent In the collinear limit $l_T \rightarrow 0$, the third gamma matrix term in the bracket has sufficiently many powers of $|\vec{l}_T|^2$ to remain finite, hence it can be neglected, since we are only interested in collinear \textit{divergences} when computing the splitting functions. It follows that the amplitude simplifies to:
\begin{equation*}
-\frac{g_B}{3 |\vec{l}_T|^2} \mathcal{M}(p-l) \left( (1-x)x \slashed{p} - (1-x) \slashed{l}_T\right) \slashed{\epsilon}(l) u(p)
\end{equation*}
%
%To make further progress, it is useful to move the gamma matrices around. We note that if we anticommute $\slashed{p}$ through $\slashed{\epsilon}(l)$ in the first term, we have
%\begin{equation*}
%(1-x) \slashed{p} \slashed{\epsilon}(l)u(p) = -(1-x) \slashed{\epsilon}(l) \slashed{p} u(p) + 2(1-x) p \cdot \epsilon(l) u(p) = 2(1-x)p \cdot \epsilon(l) u(p),
%\end{equation*}
%\noindent where $\slashed{p} u(p) = 0$ vanishes by the Dirac equation. To simplify $p \cdot \epsilon(l)$, we use the Sudakov decomposition:
%\begin{equation*}
%\epsilon(l) \cdot p = \epsilon(l) \cdot \left( \frac{l}{1-x} - \frac{l_T}{1-x} - \frac{|\vec{l}_T|^2}{1-x} \eta\right) = - 2 l_T \cdot \epsilon(l),
%\end{equation*}
%\noindent since $\epsilon(l) \cdot l = 0$ in an appropriate gauge, and the term involving $|\vec{l}_T|^2$ is suppressed in the collinear limit as it gives something finite. Hence we are left with:
%\begin{equation*}
%(1-x)\slashed{p} \slashed{\epsilon}(l) u(p) = -2 l_T \cdot \epsilon(l) u(p).
%\end{equation*} 
%\noindent Finally, note that in the collinear limit, we have $\mathcal{M}(p-l) + \mathcal{M}(xp)$ by considering the Sudakov decomposition and letting $l_T \rightarrow 0$.
Hence, the final simplified amplitude is:
\begin{equation*}
\frac{g_B}{3 |\vec{l}_T|^2} \mathcal{M}(xp) \left( 2x  l_T \cdot \epsilon(l) + (1-x) \slashed{l}_T \slashed{\epsilon}(l)\right)  u(p).
\end{equation*}
%
Taking the spin/polarisation-sum/averaged modulus squared of this amplitude, we have:
\begin{gather*}
%\frac{g_B^2}{9 |\vec{l}_T|^4} \left(\sum_{\text{pol.}}\right) \left(\frac{1}{2}\sum_{\text{spins}}\right) \mathcal{M}(xp) \left( 2 x l_T^{\mu} \epsilon_{\mu}(l) + (1-x) \slashed{l}_T \epsilon_{\mu}(l) \gamma^{\mu} \right) u(p) \bar{u}(p) \left( 2 x l_T^{\nu} \epsilon_{\nu}^*(l) + (1-x)  \epsilon^*_{\nu}(l) \gamma^{\nu} \slashed{l}_T\right) \mathcal{M}^{\dagger}(xp)\\\\
  %=
  -\frac{g_B^2}{18 |\vec{l}_T|^4} \mathcal{M}(xp) \left( 2 x l_{T\mu} + (1-x) \slashed{l}_T \gamma_{\mu} \right) \slashed{p} \left( 2 x l_T^{\mu} + (1-x) \gamma^{\mu} \slashed{l}_T\right) \mathcal{M}^{\dagger}(xp)\\\\
  = \frac{g_B^2}{9 |\vec{l}_T|^2} (1+x^2) \mathcal{M}(xp) \slashed{p} \mathcal{M}^{\dagger}(xp) = \frac{g_B^2}{9 |\vec{l}_T|^2} \left( \frac{1 + x^2}{x} \right) \mathcal{M}(xp) x\slashed{p} \mathcal{M}^{\dagger}(xp),
\end{gather*}
, where we sumed over all polarisations and used standard gamma matrix identities to simplify the
expressions in the first line.
%\noindent Note that for convenience we sum over all polarisations, including unphysical ones. There is no need to introduce ghosts since the $B$-boson comes from a $U(1)$, i.e. Abelian, model. We need to simplify the string of gamma matrices sandwiched between the $\mathcal{M}$'s.\\\\
%\noindent We use standard gamma matrix identities for computing $\slashed{q}\slashed{q}$ and $\gamma_{\mu} \slashed{q} \gamma^{\mu}$ to give:
%\begin{gather*}
%4x^2 l_T^2 \slashed{p} + 4x(1-x) l_T^2 \slashed{p} + (1-x)^2 \slashed{l}_T \gamma^{\mu} \slashed{p} \gamma_{\mu} \slashed{l}_T\\\\
%= 4x^2 l_T^2 \slashed{p} + 4x (1-x) l_T^2 \slashed{p} + 2(1-x)^2 l_T^2 \slashed{p}\\\\
%= 2 l_T^2 (1 + x^2) \slashed{p}.
%\end{gather*}
%
%Hence we are left with:
%\begin{equation*}
%\frac{g_B^2}{9 |\vec{l}_T|^2} (1+x^2) \mathcal{M}(xp) \slashed{p} \mathcal{M}^{\dagger}(xp) = \frac{g_B^2}{9 |\vec{l}_T|^2} \left( \frac{1 + x^2}{x} \right) \mathcal{M}(xp) x\slashed{p} \mathcal{M}^{\dagger}(xp).
%\end{equation*}
\noindent With this expression, we can immediately write down the cross-section contribution:
\begin{equation*}
\sigma^{(1)}(p) = \frac{1}{2s}\sum_{X} \int \frac{d^3 \vec{l}}{2l^0 (2\pi)^3} \frac{g_B^2}{9 |\vec{l}_T|^2} \left( \frac{1 + x^2}{x} \right) \mathcal{M}(xp) x\slashed{p} \mathcal{M}^{\dagger}(xp).
\end{equation*}
\noindent We can simplify the measure:
\begin{equation*}
\frac{d^3 \vec{l}}{2l^0 (2\pi)^3} = \frac{d^2 \vec{l}_T dl^3}{ 2l^0 (2\pi)^3} = \frac{d^2 \vec{l}_T dx}{2l^0 (2\pi)^3} \cdot \left| \frac{\partial l^3}{\partial x}\right| = \frac{d^2 \vec{l}_T}{2 (2\pi)^3} \cdot \frac{dx}{1-x},
\end{equation*} 
\noindent after working out the Jacobian (e.g. using the explicit expression for the Sudakov decomposition of $l$ in a particular frame, which we wrote down earlier). Performing the angular integral, we have:
\begin{equation*}
\frac{d^2 \vec{l}_T}{2 (2\pi)^3} \cdot \frac{dx}{1-x} = \frac{d(|\vec{l}_T|^2)}{4 (2\pi)^2} \cdot \frac{dx}{1-x} = \frac{1}{16 \pi^2} d(|\vec{l}_T|^2) \frac{dx}{1-x}.
\end{equation*}
\noindent Thus the cross-section is:
\begin{equation*}
\sigma^{(1)}(p) = \frac{g_B^2}{9} \int \frac{d(|\vec{l}_T|^2)}{8 \pi^2  |\vec{l}_T|^2} \int\limits_{0}^{1} dx \left( \frac{1 + x^2}{1-x}\right) \underbrace{\left( \frac{1}{4sx}\sum_{X} \mathcal{M}(xp) x\slashed{p} \mathcal{M}^{\dagger}(xp) \right)}_{\text{$\sigma^{\text{Born}}(xp)$}},
\end{equation*}
\noindent where note to transform the final factor to $\sigma^{\text{Born}}(xp)$, we require $s \mapsto sx$, since $s = 2p \cdot p' \mapsto 2xp \cdot p'$ in this case. Tidying up, we write $\alpha_B = g_B^2/4\pi$, and thus we can write the cross-section in a nicely factored form:
\begin{equation*}
\sigma^{(1)}(p) = \frac{\alpha_B}{2 \pi} \int \frac{d(|\vec{l}_T|^2)}{|\vec{l}_T|^2} \int\limits_{0}^{1} dx \ \frac{1}{9} \left( \frac{1+x^2}{1-x} \right) \sigma^{\text{Born}}(xp).
\end{equation*}
\noindent The \textit{collinear divergence} $l_T \rightarrow 0$ is now manifest, and so is a \textit{soft divergence}, $x \rightarrow 1$, which characterises the divergence that occurs when the radiated parton's energy tends to zero.\\\\
\noindent The collinear divergence is exactly the factor we want to multiply the splitting functions, so we are getting close to finding our splitting functions. First, however, we must deal with the soft divergence by the inclusion of \textit{virtual corrections}.

\noindent Before moving on to virtual corrections however, let's dispense of another issue involving the real emission of a $B$-boson. We have only considered one possible diagram that involves emission of a $B$-boson; it is rightly argued that we should include \textit{all} diagrams involving such an emission - namely, we should include a contribution from the diagrams:
\begin{figure}[H]
\centering
\begin{tikzpicture}
\begin{scope}[thick,decoration={
    markings,
    mark=at position 0.5 with {\arrow{>}}}
    ] 
\draw[dashed,postaction={decorate}] (-1,1) node[above left] {$k$}-- (0,0);
\end{scope}
\draw[thick,snake it] (0,0) -- (0.5,-1.1) node[below right]{$B$};
\begin{scope}[thick,decoration={
    markings,
    mark=at position 0.5 with {\arrow{>}}}
    ] 
\draw[postaction={decorate}] (-1,-1) node[below left] {$q$}-- (0,0);
\end{scope}
\node[circle,fill=black,inner sep=0pt,minimum size=15pt] at (0,0) {};
\begin{scope}[ultra thick,decoration={
    markings,
    mark=at position 0.7 with {\arrow{>}}}
    ] 
\draw[postaction={decorate}] (0,0) -- (1,0) node[right] {$X$};
\end{scope}
\end{tikzpicture}
\end{figure}
\noindent However, these diagrams do not contain propagators that are divergent in the collinear limit as $k_T \rightarrow 0$. At worst, they could multiply one of our former diagrams which would introduce a factor of $1/|\vec{k}_T|^2$; however, this cancels with the numerator to give something finite. Hence these graphs do not contribute in the collinear limit.

%%%%%%%%%%%%%%%
We now discuss the inclusion of virtual corrections. At this point, it may seem we have to compute more diagrams and add them to the cross-section $\sigma^{(1)}$ we found above. However, this is not actually the case - instead, we can use the simple fact that probabilities must sum to $1$ to save us.\\\\
\noindent Let's begin by writing the virtual corrections as:
\begin{equation*}
A \sigma^{\text{Born}}(p),
\end{equation*}
\noindent where $A$ is some appropriate constant. It follows that the sum of the virtual corrections and the leading order graph is given by $(1+A)\sigma^{\text{Born}}(p)$. Thus adding the virtual corrections, leading order graph and the real emission graph, we have:
\begin{equation*}
\int\limits_{0}^{1} dx \left( \frac{1}{9} \left( \frac{1+x^2}{1-x} \right) + (1+A) \delta(1-x) \right) \sigma^{\text{Born}}(xp).
\end{equation*}
\noindent We interpret the coefficient of $\sigma^{\text{Born}}(xp)$ as the possible outcomes for the initial quark: it either radiates a $B$-boson, radiates a virtual quark which later recombines with the original quark, or it does none of the above. At this order, these are the \textit{only} possibilities, and hence the probabilities of these events must sum to $1$:
\begin{equation*}
\int\limits_{0}^{1} dx \left( \frac{1}{9}\left( \frac{1 + x^2}{1-x}\right) + (1 + A)\delta(1-x) \right) = 1.
\end{equation*}
\noindent There is a problem with this equation as written though: if we immediately perform the delta function integral, we find that $A$ is equal to a \textit{divergent} expression. This isn't a problem, since we know the virtual corrections will contain divergences. But we should regulate the integral somehow. We do so by cutting off the integral for the first term at $1-\epsilon$:
\begin{equation*}
\int\limits_{0}^{1} dx \left( \frac{1}{9}\left( \frac{1 + x^2}{1-x}\right) \Theta(1 - \epsilon - x) + (1 + A)\delta(1-x) \right) = 1.
\end{equation*}
\noindent where $\Theta$ is the Heaviside step function. We can now compute the (divergent) value of $A$ that enforces this condition:
\noindent \textbf{Theorem:} For the above equation to hold, we require that the virtual contributions conspire to give
\begin{equation*}
A = \frac{1}{6} + \frac{2}{9} \log(\epsilon).
\end{equation*}
\noindent It follows that the splitting function $P_{qq}(x)$ may be viewed as a distribution:
\begin{equation*}
P_{qq}(x) = \lim_{\epsilon \rightarrow 0} \left( \frac{1}{9}\left( \frac{1 + x^2}{1-x} \right) \Theta(1 - \epsilon - x) + \delta(1-x) \left( \frac{1}{6} + \frac{2}{9} \log(\epsilon) \right) \right).
\end{equation*}
\noindent \textit{Proof:} Evaluating the integrals, the condition that probabilities must sum to $1$ can be rewritten as:
\begin{gather*}
\int\limits_{0}^{1} dx \left( \frac{1}{9}\left( \frac{1 + x^2}{1-x}\right)\Theta(1-\epsilon - x) + (1 + A)\delta(1-x) \right) = 1\\
\Rightarrow \qquad A = -\frac{1}{9}\int\limits_{0}^{1-\epsilon} dx \ \left( \frac{1+x^2}{1-x} \right) = -\frac{1}{9} \left( -\frac{3}{2} - 2 \log(\epsilon) \right) = \frac{1}{6} + \frac{2}{9} \log(\epsilon),
\end{gather*}
\noindent as required. \qedsymbol
\noindent \textbf{Theorem:} We can write the splitting function $P_{qq}(x)$ in the form:
\begin{equation*}
P_{qq}(x) = \frac{1 + x^2}{9(1-x)_+} + \frac{1}{6} \delta(1-x),
\end{equation*}
\noindent where the \textit{plus distribution} is defined by
\begin{equation*}
\int\limits_{0}^{1} dx\ f(x)_+ g(x) = \int\limits_{0}^{1} dx\ f(x) \left( g(x) - g(1) \right).
\end{equation*}
\noindent \textit{Proof:} We have
\begin{equation*}
\int\limits_{0}^{1} dx\ P_{qq}(x) f(x) = \lim_{\epsilon \rightarrow 0} \left(\int\limits_{0}^{1-\epsilon} dx \ \frac{1}{9}\left( \frac{x^2 + 1}{1-x} \right) f(x) + \frac{1}{6}f(1) + \frac{2}{9} \log(\epsilon) f(1)\right).
\end{equation*}
\noindent We note that the $f(1)$ term on its own is fine. We would like to combine the $\epsilon$'s in such a way that we can actually take the limit in the expression. We notice that 
\begin{equation*}
\int\limits_{0}^{1-\epsilon} dx\ \frac{f(1)}{1-x} = -f(1) \log(\epsilon),
\end{equation*}
\noindent hence we can take the $f(1)\log(\epsilon)$ term inside the integral in a nice way:
\begin{gather*}
\int\limits_{0}^{1} dx\ P_{qq}(x) f(x) = \lim_{\epsilon \rightarrow 0} \left( \int\limits_{0}^{1 - \epsilon} dx\ \frac{1}{9} \left( \frac{x^2 + 1}{1-x} - \frac{2 f(1)}{1 -x} \right) + \frac{1}{6} f(1) \right)\\
= \lim_{\epsilon \rightarrow 0} \left( \int\limits_{0}^{1 - \epsilon} dx\ \frac{1}{9} \left( \frac{x^2 + 1}{(1-x)_+} \right) f(x) + \frac{1}{6} f(1) \right).
\end{gather*}
\noindent Notice that the integral is now regulated as $\epsilon \rightarrow 0$, since at the upper limit the integrand becomes zero - this is the effect of the plus distribution. So we can now take the limit as $\epsilon \rightarrow 0$, and the result follows. \qedsymbol
\noindent Putting everything together then, we find that the contribution to the splitting function $P_{qq}(x)$ is given by:
\begin{equation*}
P_{qq}(x) = \frac{1+x^2}{9(1-x)_+} + \frac{1}{6} \delta(1-x)
\end{equation*}


%%%%%%%%%%%%
\subsubsection*{Contributions to $P_{qB}(x)$}
\noindent Next, let's consider the radiation of a quark from a $B$-boson:
\begin{figure}[H]
\centering
\begin{tikzpicture}
\begin{scope}[thick,decoration={
    markings,
    mark=at position 0.5 with {\arrow{>}}}
    ] 
\draw[dashed,postaction={decorate}] (-1,1) node[above left] {$k$}-- (0,0);
\draw[postaction={decorate}] (0.5,-0.8) node[right] {$\bar{q}$} -- (-0.8,-0.8);
\end{scope}
\draw[thick,snake it] (-1.5,-1.5) node[below left]{$B$}-- (-0.8,-0.8) ;
\begin{scope}[thick,decoration={
    markings,
    mark=at position 0.5 with {\arrow{>}}}
    ] 
\draw[postaction={decorate}] (-0.8,-0.8)-- (0,0);
\end{scope}
\node[circle,fill=black,inner sep=0pt,minimum size=15pt] at (0,0) {};
\begin{scope}[ultra thick,decoration={
    markings,
    mark=at position 0.7 with {\arrow{>}}}
    ] 
\draw[postaction={decorate}] (0,0) -- (1,0) node[right] {$X$};
\end{scope}
\end{tikzpicture}
\end{figure}
\noindent The amplitude for this diagram is, similar to before,
\begin{equation*}
\frac{g_B}{3(p-l)^2} \mathcal{M}(p-l) (\slashed{p} - \slashed{l}) \slashed{\epsilon}(p) v(l).
\end{equation*}
\noindent As before, we can simplify this amplitude before we take the spin/polarisation-sum/averaged modulus squared. We use the Sudakov decomposition
\begin{equation*}
l = (1-x)p + l_T + \frac{|\vec{l}_T|^2}{1-x} \eta,
\end{equation*}
\noindent which simplifies the amplitude to
\begin{equation*}
-\frac{g_B (1-x)}{3 | \vec{l}_T|^2} \mathcal{M}(xp) (x \slashed{p} - \slashed{l}_T) \slashed{\epsilon}(p) v(l),
\end{equation*}
\noindent where we have ignored all terms that remain finite as $l_T \rightarrow 0$.\\\\
\noindent We can simplify the spinor structure using the Sudakov decomposition so that all terms of order $l_T$ are apparent. Note first that we have:
\begin{equation*}
(1-x)(x \slashed{p} - \slashed{l}_T) \slashed{\epsilon}(p) v(l) = (x (1-x) \slashed{p}\slashed{\epsilon}(p) - (1-x) \slashed{l}_T \slashed{\epsilon}(p) ) v(l).
\end{equation*}
\noindent The first term simplifies using the Sudakov decomposition:
\begin{equation*}
(1-x) \slashed{p} \slashed{\epsilon}(p) v(l) = (\slashed{l} - \slashed{l}_T) \slashed{\epsilon}(p) v(l) = (2 l \cdot \epsilon(p) - \slashed{l}_T \slashed{\epsilon}(p)) v(l) = (2 \epsilon(p) \cdot l_T - \slashed{l}_T \slashed{\epsilon}(p) ) v(l),
\end{equation*}
\noindent ignoring throughout the calculation terms that give a finite contribution as $l_T \rightarrow 0$. Thus we're left with the simplified amplitude:
\begin{equation*}
-\frac{g_B}{3 | \vec{l}_T|^2} \mathcal{M}(xp) (2x \epsilon(p) \cdot l_T - \slashed{l}_T \slashed{\epsilon}(p) ) v(l).
\end{equation*}
\noindent Taking the spin/polarisation-sum/averaged modulus squared of the amplitude, we have:
\begin{equation*}
-\frac{g_B^2}{18 |\vec{l}_T|^4} \mathcal{M}(xp) (2x l_{T\mu} - \slashed{l}_T \gamma_{\mu} ) \slashed{l} (2x l_T^{\mu} - \gamma^{\mu}\slashed{l}_T  ) \mathcal{M}^{\dagger}(xp).
\end{equation*}
\noindent Simplifying the spinor structure, we get (using standard identities for the gamma matrices):
\begin{equation*}
(2x l_{T \mu} - \slashed{l} \gamma_{\mu}) \slashed{l} ( 2x l_T^{\mu} - \gamma^{\mu} \slashed{l}_T) = -4x^2 |\vec{l}_T|^2 (1-x) \slashed{p} + 4x | \vec{l}_T|^2 (1-x) \slashed{p} - 2 | \vec{l}_T|^2 (1-x)\slashed{p},
\end{equation*}
\noindent where we have again ignored any terms that give a finite contribution as $l_T \rightarrow 0$. Thus the formula we must insert into the cross-section integral is:
\begin{equation*}
\frac{g_B^2(1-x)}{9 |\vec{l}_T|^2} \left(\frac{2x^2 - 2x + 1}{x}\right)\mathcal{M}(xp) x \slashed{p} \mathcal{M}^{\dagger}(xp).
\end{equation*}

%%%%%%%%%
\noindent Inserting into the cross-section formula, we have:
\begin{equation*}
\sigma^{(1)}(p) = \frac{\alpha_B}{2\pi} \int \frac{d(|\vec{l}_T|^2)}{|\vec{l}_T|^2} \int\limits_{0}^{1} dx \ \left(\frac{2x^2 - 2x + 1}{9} \right) \sigma^{\text{Born}}(xp).
\end{equation*}
\noindent and hence we deduce that the splitting function is given by:
\begin{equation*}
P_{qB}(x) = \frac{2x^2 -2x + 1}{9} = \frac{(1-x)^2 + x^2}{9}.
\end{equation*}
\noindent In this case, there are no virtual corrections to take care of at this order.

%
\subsubsection*{Contribution to $P_{BB}(x)$}
\noindent Having found $P_{qB}(x)$, it is very easy to find $P_{BB}(x)$ using the fact that probabilities must sum to $1$. First note that at this order, the only contribution to $P_{BB}(x)$ is given by a virtual correction to the incoming $B$, namely a fermion loop on this line.\\\\
\noindent Therefore, by the fact that the probability of $B$ splitting plus the probability of the $B$ staying intact must sum to $1$, we have:
\begin{equation*}
\int\limits_{0}^{1} dx\ \left( \frac{x^2 + (1-x)^2}{9} + (1 + A)\delta(1-x)\right) = 1.
\end{equation*}
\noindent Here, $A$ denotes the virtual contribution and the $1$ denotes the contribution from the Born amplitude for $B$ to initiate the interaction. Solving this equation, we have
\begin{equation*}
A = - \int\limits_{0}^{1} dx\ \left( \frac{x^2 + (1-x)^2}{9} \right) = - \left[ \frac{x^3}{27} - \frac{(1-x)^3}{27}\right]_0^{1} = -\frac{2}{27}.
\end{equation*}
\noindent and it follows that the splitting function is given by
\begin{equation*}
P_{BB}(x) = -\frac{2}{27} \delta(1-x).
\end{equation*}


%%%%%%%%%%%%%%
\subsubsection*{Contribution to $P_{Bq}(x)$}
\noindent Finally, let's consider the radiation of a $B$ from a quark:
\begin{figure}[H]
\centering
\begin{tikzpicture}
\begin{scope}[thick,decoration={
    markings,
    mark=at position 0.5 with {\arrow{>}}}
    ] 
\draw[dashed,postaction={decorate}] (-1,1) node[above left] {$k$}-- (0,0);
\end{scope}
\draw[thick,snake it] (-0.7,-0.7) -- (0,0);
\begin{scope}[thick,decoration={
    markings,
    mark=at position 0.5 with {\arrow{>}}}
    ] 
\draw[postaction={decorate}] (-1.5,-1.5) node[below left] {$q$}-- (-0.7,-0.7);
\draw[postaction={decorate}] (-0.7,-0.7) -- (0.5,-0.7) node[right]{$q$};
\end{scope}
\node[circle,fill=black,inner sep=0pt,minimum size=15pt] at (0,0) {};
\begin{scope}[ultra thick,decoration={
    markings,
    mark=at position 0.7 with {\arrow{>}}}
    ] 
\draw[postaction={decorate}] (0,0) -- (1,0) node[right] {$X$};
\end{scope}
\end{tikzpicture}
\end{figure}
\noindent Again, the splitting function can be found using a simple probability argument. We note that 
\begin{equation*}
P_{Bq}(x) = P_{qq}(1-x) - \text{virtual corrections},
\end{equation*}
\noindent since $P_{qq}(x)$ is the probability that a quark of momentum $p$ will split into a quark of momentum $xp$ (which participates in a hard interaction) and a $B$ of momentum $(1-x)p$; whilst $P_{Bq}(1-x)$ is the probability that a quark of momentum $p$ will split into a $B$ of momentum $xp$ (which participates in a hard interaction) and a $B$ of momentum $(1-x)p$. The only difference is the participant in the hard reaction, whose only effect on the splitting function is to determine whether virtual corrections are necessary or not. Hence the identity follows.\\\\
\noindent It follows that
\begin{equation*}
P_{Bq}(x) = \frac{1}{9} \left( \frac{1 + (1-x)^2}{1 - (1-x)} \right) = \frac{1}{9} \left( \frac{1 + (1-x)^2}{x} \right).
\end{equation*}

